Improving the TENOR of Labeling: Re-evaluating Topic Models for Content Analysis

Topic models are a popular tool for understanding text collections, but their evaluation has been a point of contention. Automated evaluation metrics such as coherence are often used, however, their validity has been questioned for neural topic models (NTMs) and can overlook a models benefits in real world applications. To this end, we conduct the first evaluation of neural, supervised and classical topic models in an interactive task based setting. We combine topic models with a classifier and test their ability to help humans conduct content analysis and document annotation. From simulated, real user and expert pilot studies, the Contextual Neural Topic Model does the best on cluster evaluation metrics and human evaluations; however, LDA is competitive with two other NTMs under our simulated experiment and user study results, contrary to what coherence scores suggest. We show that current automated metrics do not provide a complete picture of topic modeling capabilities, but the right choice of NTMs can be better than classical models on practical task.

==> scripts/style-check/bad-words <==
utilize              % phrase "use" http://www.bartleby.com/64/C003/0294.html
utilizes             % phrase "uses" http://www.bartleby.com/64/C003/0294.html
utilized             % phrase "used" http://www.bartleby.com/64/C003/0294.html
utilizing            % phrase "using" http://www.bartleby.com/64/C003/0294.html
leverage             % phrase "use"
abstraction          % phrase this is often used poorly?
fashion              % phrase hrm.
[dw]on't             % spelling do not or will not.
behavioral           % spelling I'm convinced we don't use this word properly.
we'll                % spelling we will
we've                % spelling we have
[^r][^c][^h] impact  % phrase "consequences", "effect", "result", though nsf likes "research impact"
tackle               % phrase "tackle" (a problem) is wimpy for "solve" or a tired metaphor for "address a challenge".
thusly               % phrase "thus" or "this way" or "like this" http://www.bartleby.com/64/C003/0282.html
transpire            % phrase "happen" 
so-called            % phrase can be abused; it's negative.
necessitate          % phrase require.
necessitated         % phrase required.
necessitates         % phrase requires.
loosing              % spelling you almost certainly mean "losing".  use "loosening" otherwise.
aforementioned       % phrase too pretentious.
important to         % phrase "valued by"?
notion               % phrase avoid this weak phrase. (thanks brian bershad!)
achieve(s)?\s        % phrase models don't achieve anything, only use for humans
reasonably           % phrase hedging


==> scripts/style-check/common-typos <==
a the                % phrase double article
 pt                  % syntax ? I guess avoid straggling pt's that escape tex?
[ ],                 % syntax whitespace before comma seems wrong.
Figure Figure        % phrase pizza pizza.
[ ]-[ ]              % syntax a hyphen surrounded by space should probably be an emdash '---'
[0-9]-[0-9]          % syntax use an endash '--' for ranges
[0-9]ms              % syntax put a space between the number and the unit.
[^egs]\. [a-z]       % syntax a period usually ends a sentence, and sentences should start with a capital; doesn't apply for i.e.,
\.  [a-z]            % syntax a period usually ends a sentence, and sentences should start with a capital; "i.e." should have a comma following.
[a-z]\.\.            % syntax double period is rarely right, use \ldots for ellipsis
[^\\]"               % syntax use fancy quotes
\beg\.               % syntax should be e.g. as in "examples given"
from to\b            % phrase haven't used this properly.
help help            % phrase double word, that probably means the author paniced
of of                % phrase apparent double word.
the affect           % phrase should probably be 'the effect'
the the              % phrase apparent double word.
there too few        % phrase there are too few?
was not was          % phrase pretty much a joke if this gets matched.
we we                % phrase it would be oi oi in french, I guess.
with on              % phrase probably wrong.
with with            % phrase apparent double word.
[\n ]--[\n ]         % syntax that's an en-dash, you want an em-dash: "---"
my my                % phrase unlikely that's what you want, at least without a comma. (doesn't work across newlines)
>From                % syntax be careful when you email .tex files.  I've seen this slip through into submissions.
e\.t\.c\.            % syntax it's et cetera; use etc.
such as like         % phrase pick one
<<<<<<< .            % syntax CVS conflict!
=======              % syntax CVS conflict!
>>>>>>> [0-9]        % syntax CVS conflict!
e\.g\.[\n ]          % syntax should be followed with a comma, as e.g. can be read as "for example" (thanks JZ!)
i\.e\.[\n ]          % syntax should be followed with a comma, as i.e. can be read as "that is" (thanks JZ!)
[ ]\.[\n ]           % syntax stray period?
further more         % phrase one word: furthermore
safe guard           % phrase one word: safeguard
that be              % phrase mistake.
can not              % phrase cannot
only only            % phrase double word
is is                % phrase double word.
they shows           % phrase argh, mistake.
less that than       % phrase typo damage
from from            % phrase double word score
in in                % phrase "in" (common mistake)
not not              % phrase argh.
it it                % phrase argh.
to illicit           % phrase "to elicit" -- illicit is always an adjective.
c\.f\.               % phrase actually, it's cf., and you'd like cf.\ (backslash space)
this lead to         % phrase "led to" if past tense, "leads to" if present.
on on                % phrase double word.
has is               % phrase choose
description their    % phrase saw this, clearly wrong.
including:  % syntax I prefer no colon after including, which already says a list is coming.
[a-z]\([A-Z]  % syntax put a space before parens, even when introducing acronyms.
without and without % phrase saw this.
can be result       % phrase saw this typo.



==> scripts/style-check/foolish-phrases <==
(quite|more|very|most) unique    % phrase unique is.
(quite|more|very|most) abstract  % phrase abstract is.
tangible view                    % phrase mix that metaphor some more.
for e\.g\.                       % phrase e.g. includes "for".
begs the question                % phrase unless you're very clever: "raises the question": http://alt-usage-english.org/excerpts/fxbegthe.html
high rate of speed               % phrase local news-speak.
especially necessary             % phrase 'especially important', necessary may be an absolute like unique.
how will it effect % phrase you likely meant "affect"
how it will effect % phrase you likely meant "affect"
insure proper performance % phrase "ensure"
especially true                  % phrase 'especially important', true may be an absolute like unique.
to affect change                 % phrase "effect" change;  I read this on a poster.
higher results                   % phrase maybe higher performance or higher values.
is more general then the         % phrase probably "than"
upper bounding                   % phrase "limiting" or "setting an upper bound on"
in principal                     % phrase likely, "in principle"
literally like                   % phrase literally means no simile.  
design principal  % phrase likely, "design principle" 
different from 	    	   	 % phrase unlike

==> scripts/style-check/latex-checking <==
\{\\em [^\}]*[^\}\/]\}[:]    % syntax use \emph{} or explicit italic correction {\em foo\/}
\{\\em [^\}]*[:\.,]\}        % syntax punctuation at the edges of italic text is not italicized
[A-Z]{2,10}\.[ ]*[\n ][ ]*[A-Z]  % syntax intersentence spacing should be used if a sentence ends with an acronym: "FOO\\@."
\\etal[^{]                   % syntax it's good practice to use \etal{} to avoid bad spacing
\\caption\[[^\]]*[^\.]\]     % syntax short caption should end with a period.
\\caption\[.*CCDF.*\]        % syntax short caption should not include graph type.
\\caption\[.*CDF.*\]         % syntax short caption should not include graph type.
\\caption\[.{0,25}\]         % syntax short caption should not be too short.
th century                   % syntax use textsuperscript
[ ]---[ ]                    % syntax the em-dash should be right up against the words.
[ \n]---[ \n]                % syntax the em-dash should be right up against the words.
^---[ \n]                    % syntax the em-dash should be right up against the words.
[ \n]---$                    % syntax the em-dash should be right up against the words.
[ \n]--[ \n]                 % syntax the en-dash should be between numbers.
^--[ \n]                     % syntax the en-dash should be between numbers.
[ \n]--$                     % syntax the en-dash should be rbetween numbers.
,[~ ]\\etal                  % syntax no comma before etal (unless Smith, Martinez, \etal)
\\etal\{\}'s                 % syntax eew.
\\(sub)?section\{[A-Z][^}]*[ ][a-z]{5,40}[^}]*\} % syntax subsection headers should be initial capped.
\\(sub)?section\{[A-Z][^}]*[^:][ ]{1,}(With|A|An|Is|And|For|To|The)[ ][^}]*\} % syntax some words needn't be capitalized
[ ]\\footnote                % syntax no space before footnote.
\\footnote\{.*\}.            % syntax footnotes after punctuation
,,                           % syntax double comma is unlikely to be intentional.
cf\.[^\\]                    % phrase cf. should get an escaped space "\ "
et al\.[^\\]                    % phrase et al. should get an escaped space "\ "
[<>]  % syntax a less than or greater than outside math mode shows other characters.
in (section|table|figure) \\ref % phrase should have ~ before ref
section~\\ref % capitalize capitalize section when saying Section 6.
table~\\ref % capitalize capitalize section when saying Table 6.
figure~\\ref % capitalize capitalize section when saying Figure 6.
\\(sub)?section\{Intro\} % syntax spell it out.
,''                          % syntax punctuation outside quotes
\.\.\.                       % syntax use \dots

==> scripts/style-check/my-rules <==
#  such may be abused to blacklist certain words even spelled correctly.
# capitalize is case sensitive, and also bracketed by non-word.
# phrase and spelling are case insensitive, but bracketed by non-word characters.
# syntax is case sensitive but not bracketed by non-word; probably best if used with regexes.
\bet al\.[^}]        % syntax use the \etal{} command instead. (or write one to italicize)
\bet\. al\.          % syntax use the \etal{} command, "et" needs no dot (et alii). (or write one to italicize)
\bc\.f\.\b             % syntax should be cf. for "confer" (latin for compare)
\b$i\)[^$]              % syntax leave the paren in math mode -- should be $i)$
\b$ii\)[^$]             % syntax leave the paren in math mode -- should be $ii)$
\b$iii\)[^$]            % syntax leave the paren in math mode -- should be $iii)$
\b$iv\)[^$]             % syntax leave the paren in math mode -- should be $iv)$
\b$v\)[^$]              % syntax leave the paren in math mode -- should be $v)$
\ban [b-df-gj-np-tv-z] % syntax probably meant to use "a" instead of "an", though there are exceptions.
\ban [B-DF-GJ-NP-TV-Z][^A-Z/] % syntax probably meant to use "a" instead of "an", though there are exceptions (like acronyms).
\b[Aa] [aeiouAEIOU](?!se|ni|A|ur|RL|ti|ne|DP) % syntax probably meant to use "an" instead of "a", though there are exceptions. (user, useful, AA, unified, uniform, unique, Europe, one, UDP; n/a doesn't work, so use {n/a})
This allows           % phrase tie more explicitly: This (x) allows...
we find               % phrase omit "we find"
we found              % phrase omit "we found"
try and               % phrase "try to", though if you're using try as a noun in a compound sentence, this rule is wrong.
impact of             % phrase not a useful metaphor; try evaluation, success, effect, value.
including [^\.]*etc\. % syntax "including" tells of a non-exclusive list, so "etc." is redundant.  This rule will misfire if you have two lists in your sentence, but you shouldn't do that either. ;)
includes [^\.]*etc\.  % syntax "includes" tells of a non-exclusive list, so "etc." is redundant.  This rule will misfire if you have two lists in your sentence, but you shouldn't do that either. ;)
and etc\.             % phrase come on. learn some latin.
AT&T                  % syntax you poor thing, this won't compile.
doesn't               % phrase be formal.
be occur              % phrase what happens when I'm indecisive about what follows "can"
up until              % phrase "until"
one or more           % phrase probably redundant -- nonzero is probably implied.
is comprise(d|s) of   % phrase you probably mean "is composed of" because "comprises" is more a synonym for "contains" 
will be significantly different % phrase "will differ significantly" for active voice
More importantly,     % phrase probably means the order is wrong: put important stuff first.
todo                  % ignoredcommand
texttt                  % ignoredcommand
jbgcomment              % ignoredcommand
lkfcomment              % ignoredcommand
due to space constraints % phrase don't whine.
this paper % phrase can be ambiguous if talking about someone else's paper whether you mean the one youre writing or the one you're talking about..
the above             % phrase horrible phrase that must be expunged.  you might use "these" instead, but best to make the sentence stand alone.
referred to above     % phrase "these".
(all|the|of) [0-9][ ] %  phrase use words for numbers in phrases.
clearly shows         % phrase "clearly" is usually much.
grows larger          % phrase is "grows smaller" possible?  grows.
guarantee as much as possible % phrase then not really a guarantee "provide"
affects negatively   % phrase "hurts" or "harms"
rely upon % phrase rely on is good enough
relies upon % phrase relies on is good enough
record route packets? % phrase hyphenate record-route packets
record-route; % phrase leave record route alone if not modifying something else
we accomplish this  % phrase verbose way to get active voice.
refers to the % phrase you're being wimpy in the definition.  use "is"
\\emph\{[a-zA-Z ]*\} refers to % syntax you're being wimpy in the definition.
loss off % phrase loss of?
this could % phrase this "what" could
with that has % phrase probably just one
simply % phrase probably isn't.
to get to % phrase "to reach"?
latency benefit % phrase reduction
latency improvement % phrase reduction
shed insight % phrase 'shed light' would seem the metaphor.
increasingly more % phrase redundant
I\.e\. % syntax starting a sentence with i.e. is just ugly.
E\.g\. % syntax starting a sentence with e.g. is just ugly.
in the large % phrase if large is a noun, bad.  if it's an adjective, fine.
encapsulates with % phrase seen it, don't know what it means.
when working with % phrase just say "with"
it is true that	  % phrase usually can delete
LDA % phrase convention put in small caps
(F|f)indings (show|indicate|suggest)	% phrase delete or make more specific

==> scripts/style-check/networking-research <==
IPs                  % phrase should be IP addresses
[Rr]ate-limits       % spelling "rate limits" has no hyphen, only "rate-limited"
best effort          % phrase hyphenate best-effort service.
deliver route        % phrase jargon redundancy
euclidean % capitalize Euclidean.
interdomain          % spelling inter-domain
internet             % capitalize unless talking about an internet other than the Internet
intradomain          % spelling intra-domain
log-normal           % spelling lognormal is one word.
pareto               % capitalize
ttl                  % capitalize
weibull              % capitalize proper name.
PoP                  % syntax I think POP looks less annoying.
PoPs                 % syntax I think POP looks less annoying.
http[ ]              % capitalize capitalize HTTP.
linux                % capitalize capitalize Linux
Internet[^\.]*Internet % syntax avoid Internet twice in the same sentence?
zipf                 % capitalize capitalize the guy's name.


==> scripts/style-check/passive-voice <==
it is possible to                   % phrase passive voice, try: "can"
are identified by                   % phrase passive
is shown                            % phrase passive.
is not included in                  % phrase maybe this is passive
there (are|is) [^\.:;]* (that|in)   % phrase maybe this is passive
can be evaluated                    % phrase avoid passive: I evaluated
can be observed                     % phrase avoid passive: are visible
# is needed                         % phrase passive voice
is used to                          % phrase go active voice, or subsititute "helps"
(are|were) needed[^\?]              % phrase passive voice
(is|are) presented in               % phrase "appears in", or reword to avoid passive voice
it is possible that                 % phrase "may"
(is|are) (depicted|illustrated|sketched) in  % phrase thats passive voice
(is|are) shown in                   % phrase "shows"
as can be seen in                   % phrase X shows that Y.
there needs to be                   % phrase passive voice in a bad way.
was designed                        % phrase passive voce.
it may be                           % phrase passive "it"
it is important that                % phrase passive; replace with X is important because Y.


==> scripts/style-check/verbose-phrases <==
a large number of                   % phrase you mean "many"
a substantial number of             % phrase how substantial?  most?  or just enough that can't be ignored?
an insufficient number of           % phrase "too few"
a significant number of             % phrase one is significant.   consider "prohibitive" if the number is sufficient to be problematic.
a number of                         % phrase getting the verb agreement for this useless phrase is tricky.
a number of different               % phrase use "different" (should have a high score)
a small number of                   % phrase you mean "few"
a low number of                   % phrase you mean "few"
a relatively low number of                   % phrase you mean "few"
actually                            % spelling probably doesn't add
to an extent                        % phrase you can probably remove
and instead                         % phrase replace with but?
be done                             % phrase if "X of Y can be done", try "Y can be Xed"; it's already passive voice.
combining multiple                  % phrase as opposed to "combining one?"
aggregating multiple                % phrase "aggregating"
do this                             % phrase probably verbose if you use a pronoun for what you're doing
exists[ ]                           % phrase probably no better than "is", but end of sentence may be unavoidable?
if it is to                         % phrase should be "to" (usually followed by "be X")
if they are to                      % phrase should be "to" (usually followed by "be X")
in general                          % phrase unless matched with "in specific," this is usually useless; perhaps "overall"
in order to                         % phrase remove "in order" and get "to"
in the past                         % phrase past tense is likely enough.
in the way of                       % phrase should be "as"
counting the number of              % phrase counting.  dude.
is permitted to                     % phrase "may"
largely opaque                      % phrase largely does not modify opaque
makes a new                         % phrase should be "creates"
may not chose                       % phrase "may not" is future tense; "chose" is past.
one should note                     % phrase just write it.
note that                           % phrase is the rest of the paper less notable?
Note, that                          % syntax not only should you not "note that", no comma after note.
we note                             % phrase is the rest of the paper less notable?
note however that                   % phrase is the rest of the paper less notable?
it is important to note             % phrase is the rest of the paper less notable?
really                              % phrase probably doesn't add; if you think it does, use "r{}eally" -- don't change to 'in fact'
in fact				    % phrase cut
rigorously                          % spelling probably doesn't add, and I rarely do anything with rigor
the way in which                    % phrase should be "how" or ""
the manner in which                 % phrase should be "how" or ""
value stems                         % phrase value is derived or offered, I think.
time at which                       % phrase very likely "when"
place at which                      % phrase very likely "where"
at the time                         % phrase very likely "when"
reduced number of                   % phrase very likely "fewer" or maybe maybe "less"
is present in                       % phrase present is probably redudant, try "is in"
they all                            % phrase maybe "all xs" would be better.
easy to do                          % phrase "feasible" or "practical" might be better.
is going to                         % phrase "will".
are going to                        % phrase "will".
getting                             % phrase probably "receiving" or "querying"
those are                           % phrase see if "those X are" is clearer?
design is motivated                 % phrase "inspired by" is probably better than "motivated" for design
locations throughout the world      % phrase drop "throughout the world"
e.g., as opposed to                 % phrase if you're giving examples, you're not talking about what isn't.  drop "e.g."
in addition, we also                % phrase remove either "also" or "in addition"
other related issues                % phrase probably remove "other"
the aforementioned                  % phrase "these xs" or "this x" would be less snooty
center around                       % phrase (cook) a center is a point: "center on" is okay.
could care less                     % phrase (cook) 'really? how much less could you care?' (should be couldn't)
grouped together                    % phrase redundant.  "grouped" alone should suffice.
put together                        % phrase long: "construct" "build" or "assemble"
consistent with each other          % phrase redundant.  "consistent" suffices.
be accomplished with                % phrase try "requires" "uses" "needs"?
the lack of knowledge of            % phrase would "X is unknown" work better?
gets to know                        % phrase you mean "learns"
trying to look like                 % phrase you mean "acting", "emulating", or "mimicing"
has got to be                       % phrase "must be"
got                                 % phrase try "became" "received" ?
gotten                              % phrase try "helped" ?
live in a vacuum                    % phrase a tired metaphor that makes me want to vomit.
positive impact                     % phrase try "benefit"
negative impact                     % phrase try "harm" or "consequences"
adverse impact                      % phrase try "harm" or "consequences"
adversely impacting                 % phrase try "harming" or "hurting"
discuss the issues of               % phrase could probably drop "the issues of" unless there's a list
the presence of                     % phrase not far from 'is', 'has', etc.
does not allow                      % phrase consider "forbids" or "prohibits"
and/or                              % phrase just say or.
there is the potential to           % phrase just say may.
there is the possibility that       % phrase just say might.
can be achieved                     % phrase maybe not so good?
find out                            % phrase perhaps determine?
in the absence of                   % phrase perhaps without?
in the presence of                  % phrase perhaps with?
set up                              % phrase perhaps create, configure, or initialize
in the face of                      % phrase can be overused.  try despite?
several times (at|of)               % phrase discouraged by Kurt.
a large degree of                   % phrase ick.
we start by first                   % phrase redundant. ("first, we" or "we start by").
in general, they are usually        % phrase redundant.
refers to the notion                % phrase define your term precisely if possible.
a significant amount of             % phrase probably just "significant"
real practical                      % phrase as opposed to imaginary practical?
people that are                     % phrase use people who are?
additional detail that we add       % phrase as opposed to additional detail that we subtract?
in some cases and not in others     % phrase "in some cases"
it is known that                    % phrase just say it.
caused due to                       % phrase "caused by"
a result of the fact that           % phrase "caused by"
results (indicate|show|suggest)     % phrase drop
research (indicates|show|suggest)   % phrase drop
can be attributed to the fact that  % phrase "is because"
a large set of                      % phrase probably don't care that it is a set.
a small set of                      % phrase probably don't care that it is a set: use 'a few'
provides a look at                  % phrase (timid) probably mean "shows".
in most cases                       % phrase "usually"
continue into the forseeable future % phrase "continue".
for the forseeable future           % phrase drop.
fail to successfully                % phrase "fail to" is sufficient.
Clearly,                            % syntax starting a sentence with clearly confuses me.
in different continents             % phrase ON different continents, IN different countries
(we|to) handle                      % phrase use a more specific verb like address, treat, solve
handling                            % phrase use a more specific verb like addressing, treating, solving, mitigating (unless handling errors or exceptions)
For the purposes of                 % phrase "For"
We observe that                     % phrase drop.
some degree of                      % phrase "some"
in the problem of                   % phrase (contributed by rap)
conclude several things             % phrase make (draw) several conclusions
extra bonus                         % phrase "bonus"
added bonus                         % phrase "bonus"
it is important to emphasize that   % phrase use diction to emphasize.
it is possible that                 % phrase "x may y"
caused due to                       % phrase "caused by"
recent work by                      % phrase could maybe be dropped, as the cite will include the date.
identify the location of            % phrase "find"
that go across                      % phrase "that cross"
ideally, we would like              % phrase "we would like"
enabling the ability to             % phrase "supporting" or "allowing" or "permitting"
absolutely essential                % phrase essential is.
we essentially do                   % phrase essentially is a poor adverb.  "The essence of our algorithm is a..."
Essentially,                        % phrase maybe "In essence," but could also be removed.
In this section (we|I)              % phrase "In this section, we", or "In this section, I"
essentially all                     % phrase "most"
past experience                     % phrase "experience" http://www.cmu.edu/styleguide/trickywords.html
particulary difficult primarily     % phrase simplify
intuition about why                 % phrase "intuition as to why"
Recall from above                   % phrase "recall"
Further, (I|we) will also           % phrase drop further or also
respectively                        % phrase unneeded.
in terms of                         % phrase don't need this.
the extent to which                 % phrase "how much"
make sure                           % phrase "ensure"
make up                             % phrase "constitute" "compose"
make use of                         % phrase "use"
make a decision                     % phrase "decide"
make a guess                        % phrase "guess"
since that time                     % phrase "since then"
choices to make                     % phrase "choices"
certain limitations                 % phrase what does 'certain' add to limitations?
will [a-z]* in the future           % phrase "will"
business entities                   % phrase "businesses"
rely primarily on                   % phrase "primarily" weakens "rely".  perhaps just "use" would be simpler.
has the potential to                % phrase can
have not yet developed              % phrase "have yet to develop"
to be effective,                    % phrase probably redundant.
provide information about           % phrase "tell how" "reveal" "expose" "disclose"
are different,                      % phrase "differ"
have already been                   % phrase "have been"? "were"?
as appropriate                      % phrase not needed?
only rarely                         % phrase "rarely" is probably enough.
is effective at                     % phrase "can"
foremost among them is              % phrase "foremost is" would be shorter.
those that have no                  % phrase those without
that have no                        % phrase "without"?
a variety of diverse                % phrase redundant
be highly valuable in               % phrase simplify.
the overall goal                    % phrase 'the goal'
sometimes an? [a-z]+ will           % phrase an x may
this is perhaps because             % phrase this may be because
adding an additional                % phrase redundant
IP protocol                         % phrase redundant
works well                          % phrase be more specific.
something                           % phrase could eliminate.
to keep from                        % phrase "to avoid"
[\.,] since (!then)                 % phrase probably you mean "because" unless you're talking about time. -- "has since" is okay.
performance characteristics         % phrase rare that characteristics adds.
takes into account                  % phrase considers
specify particular                  % phrase if specifying, particular should be redundant.
prototype implementation            % phrase "implementation" is redundant.
given a particular                  % phrase "given a" is probably enough
described in detail (in|below)      % phrase use "detailed"
relatively more                     % phrase more is already relative.
focus primarily on                  % phrase bad metaphor: subject of focus is singular.
primary focus                       % phrase bad metaphor: subject of focus is singular.
relatively more                     % phrase more is already relative.
gives [a-z]+ [a-z]+ information about % phrase use "tells" x
gives [a-z]+ information about      % phrase use "tells" x
an important question to ask is     % phrase just ask it.
an interesting thing                % phrase avoid saying something is interesting.  if you have to say it, it isn't.
checks to see if                    % phrase "checks" or "determines"
have an effect on                   % phrase "affect"
an important question to ask is     % phrase just ask it.
an interesting thing                % phrase avoid saying something is interesting.  if you have to say it, it isn't.
checks to see if                    % phrase "checks" or "determines"
we can see                          % phrase "we can see" isn't formal enough.
still remain                        % phrase "remain".
change over time                    % phrase "change"
turn into                           % phrase "become"
looking back in retrospect          % phrase pick.
ensures that there will be no       % phrase "prevents"
does have                           % phrase "has"
first step toward this              % phrase "toward this" can probably be dropped.
can potentially be                  % phrase "might be", or just "can be"
obviates the need for               % phrase just obviates x, not obviates the need for x.
it is indeed                        % phrase "it is", though still passive.
planning in advance                 % phrase when else might you plan?
a lot of                            % phrase "many"
keep in mind                        % phrase "consider" (or drop)
it is clear that                    % phrase if clear, you don't have to say it.
especially true                     % phrase true is an absolute, can't be especially true.
making it increasingly difficult    % phrase preventing, discouraging, impeding, blocking, slowing...
is potentially                      % phrase "may be"
have been [a-z]* in the past        % phrase 'in the past' is redundant with tense.
amount of time  % phrase "duration"
should ideally % phrase "should"
are of great benefit to % phrase "help" or "aid"
are of benefit to % phrase "help" or "aid" or "promote"
important here % phrase consider "relevant"
while at the same time % phrase "while" is enough.
are able to % phrase can
subvert the proper operation of % phrase subvert
speed slow % phrase speed is probably redundant.
of size no smaller than % phrase "of size" is probably redundant
of size no larger than % phrase "of size" is probably redundant
of size smaller than % phrase "of size" is probably redundant
of size larger than % phrase "of size" is probably redundant
might potentially % phrase "might"
in the context of % phrase "in" avoid, if possible.
increase the amount of % phrase probably just increase.
show the difference between % phrase compare
in addition, we also % phrase pick.
overhead efficiency % phrase huh?
have an effect on % phrase "affect"
have a signficant effect on %  phrase "affect"
we find % phrase can usually be removed
this suggests % phrase remove or make more precise
effective for providing	   	 % phrase remove
we performed a                   % phrase just use the verb directly
we perform a                     % phrase just use the verb directly
were able to                     % phrase could
are able to                      % phrase can


==> sections/50-experiment_simu.tex <==
%% Zongxia

%% Comment: Should I also introduce our results for Bertopic, Supervised \abr{ctm}, ETM, LLDA in the simulated experiment section
Before conducting a real-world user study, we run simulated experiments on both datasets to validate the classifiers' learning curve on purity, \abr{ari}, and \abr{anmi} is as expected.
% classifier's per formance across our four distinct groups
% , ensuring models function as intended.


\begin{figure}
    \jbgcomment{Why is this not centered?}
    \hspace*{-0.35cm} % Adjust this value as needed to shift the figure
    \includegraphics[scale=0.1]{figures/bill_synthetic1.pdf}
    \caption{Simulated experiment on the median evaluation within each group of classifier's purity, \abr{ARI}, \abr{ANMI} verses number of documents labeled over 15 runs}
    \label{fig:synthetic}
\end{figure}


\paragraph{Training Topic Models}
We preprocess the dataset by tokenizing, filtering stopwords; we use a tf-idf threshold of 3 t o remove rare and too common words. 

For \abr{lda} and \abr{slda}, we use the Tomotopy library ~\cite{tomotopy}, which uses Gibbs sampling to train classical topic models. 
% We train ~\cite{kitty_ctm} CombinedTM, a subclass of \abr{ctm}, for our simulated study. 
% To be consistent among the three models, 
% We choose the number of topics $K$ based on the following criteria: the number of topics should not be too larger to overwhelmed the users; the number of topics should not be too small so users see repetitive topics when labling a document too often; overall coherence difference among the three models should be fairly small; the distribution of documents for each topic is farily balanced. 
% We did a grid search to choose the number of topics and 
To have a fair comparison between two datasets, we chose $K=35$ topics for all three topic models in our group, which optimized average coherence. For \abr{lda} and \abr{slda}, we use term weight scheme ONE~\cite{termWeight}. \abr{slda} takes more extra hyperparameters than \abr{lda} does, for \abr{slda}, we also use binary type response variables to indicate user input labels. Otherwise, \abr{lda} and \abr{slda} use the default hyperparameter values. \abr{slda} initially does not take in any response variables. We train \abr{lda} and \abr{slda} with 2000 iterations, until a smaller change of log-likelihood and NPMI coherence. 

For \abr{ctm}, we use SBERT \texttt{paraphrase-distilroberta-base-v2} to fetch sentence embeddings for the dataset, then concatenate them with BoW representation. We used \textit{CombinedTM}~\cite{kitty_ctm} with a 768 contextual size, with $K=35$ topics, and trained it with 250 epoches. 


\paragraph{Classifier Initialization and Features}
Since users are more likely to create more granular label specifications for each document. We used sublabels as pseudo user-entered labels, while using the more general labels as our gold standard. 

We use \texttt{sklearn} SGD as our classifier for active learning document selection.\footnote{We use hyperparameters: loss='log\_loss', penalty='l2', tolerance=10e-3, random\_state=42, learning\_rate='optimal', eta0=0.1, validation\_fraction=0.2, and alpha=0.000005.} We transform our raw dataset using unigram tf-idf as input features for the classifier. For \abr{lda}, \abr{slda}, and \abr{ctm} groups, we also concatenate topic probability distributions for all the documents with unigram tf-idf features that also encodes topic information to the classifier. Since the classifier requires at least two classes to be fitted, we pick random documents and use sublabels as surrogate user input labels and activate the preference function until the classifier at least sees two class labels. We use incremental leaning~\cite{incrementallearning} to fit and update the classifier, retaining originally learned parameters.\footnote{There are two exceptions we reinitialize the classifier: if a new label class is introduced to the classifier, we reinitialize the classifier and train it with labeled documents; if \abr{slda} is updated with surrogate response variables, we rebuild the features by concatenating tf-idf features with new topic probability distributions, and restart the classifier with new features.} The clustering quality is assessed by the classifier's predictions with the more general labels.



% \paragraph{Experiment Result}
% \textbf{Also add GPT 3.5-turbo results here if need to label 500 documents.}

% \mzcomment{Reran slda for 20newsgroup and is still updating. Will include it in figure 1 only done training}

\paragraph{Simulated Experiment}
Upon analyzing the document lengths in our dataset, we deduced that, considering individual reading speed variances, a user can feasibly label between 90 to 300 documents within an hour. For our simulated user study, we automatically run our algorithm for each group to input labels for 400 documents, constantly updating the classifier for every document labeled, and \abr{slda} for every 50 documents labeled. Each group underwent 15 iterations of the experiment. For consistency, we aggregated the results by taking the median value for each document in each group. 
% In this setup, subtopics acted as surrogate user labels, while the major topic served as the gold standard. As the study progressed, we incrementally introduced surrogate labels to classifiers based on preference functions. 


\paragraph{Validity of Simulated Experiments}
Of all the methods, \abr{ctm} consistently does better on purity, \abr{ari}, and \abr{anmi}. This underscores \abr{ntm}s can generate topic probability features that do better on classification. Such features, rooted in pretrained embeddings, are perceived by compact machine learning models as more intuitive than the generative topic probabilities yielded by classical models like \abr{lda} and \abr{slda}. \abr{slda}, on the other side, is worse than \abr{lda}. The classifier without topic information falls short behind classifier with topic information. 

Our simple simulated experiments serve as a reliable proxy, allowing us to expect similar trends when actual human labeling is in play, and to track the evolution of classifier predictions as more documents are labeled over time. However, we acknowledge that relying solely on simulated evaluation metrics has its limitations. The classifier does not take into account of using topic keywords and topic overview to create labels. Other factors including fatigue, and loss of attention might also affect the quality of labels created by real user. Such metrics also do not capture the complete essence of user preferences, especially concerning the keywords produced by topic models, the highlighted keywords, or the specific documents recommended by the preference function. 



%% Zongxia

==> sections/900-discussion.tex <==
%% Zongxia
% \paragraph{Qualitative Analysis}
% We examined users' comments on the tool. 


\paragraph{User response time} In table \ref{table:user_response_time}, we present the average and median labeling times in seconds per document for users in each group. The NA group exhibits the shortest duration, while the NONE group takes the longest. Participants spend more time labeling without the aid of topic model keywords and highlights. While neural topic models can sometimes produce overly specific or nonsensical keywords beyond the top \(N\) (where \(N\) is dataset-dependent)~\cite{put citation}, this does not seem to hinder users' labeling experience, likely because their judgments are based on the top keywords. Additionally, highlights above a 0.05 threshold for documents in LDA, sLDA, CTM could also influence the labeling speed. Furthermore, based on automatic evaluation metrics and table \ref{table:no_topic_feature_metrics}, classical LDA does not display a significant advantage over NTM in a human-in-the-loop application, both on accelerating the labeling process and enhancing label quality.


\begin{table}[ht]
\centering
\begin{tabular}{l c c}
\hline
 & Mean & Median \\
\hline
\hline
NONE  & 30.18 & 18.0\\
\hline
LDA  & 24.16 & 15.5\\
\hline
sLDA & 22.86 & 16.0\\
\hline
CTM & 21.19 & 11.0\\ % Ensure this notation is intentional
\hline
\end{tabular}

\caption{Mean and median time participants spent labeling a document for each group in seconds}
\label{table:user_response_time}
\end{table}

% \paragraph{User Rating Scaling} In our post-study survey, participants rated the mental demand of the task on a scale of 1 to 7. We interpreted ratings above 4 as indicating above-average challenge, and those below 4 as signifying low challenge. In the NONE group, two-thirds (2 out of 3) found the task mentally demanding. For the sA group, 80\% (4 out of 5) considered it challenging, with half of them assigning a neutral score of 4. This suggests that continually updating sLDA, introducing new topics, and altering keywords can potentially increase the cognitive load for participants. They might need time and mental energy to adapt to these new changes. In the LDA group, 40\% (2 out of 5) found it demanding, whereas one participant felt it required no mental effort, rating it a mere 1. In the CTM group, 60\% (3 out of 5) considered the task mentally demanding. In all the groups, except LDA, the majority of the participants found the task to be mentally demanding. This could suggest that the one hour long session task inherently requires a degree of cognitive effort, while LDA might produce more sensible topic keywords that reduce user cognitive load.

% Participants were asked to rate their confidence in the labels they assigned to the documents on a scale of 1 to 7, with higher scores indicating greater confidence. We interpret scores above 4 as above-average confidence. In the LDA Group, all participants indicated a uniform sense of above-average confidence in their labeling. For the sLDA Group, while the majority rated a confident score of 6, one participant expressed a lower confidence of 3. This disparity might hint that updating models can occasionally undermine user confidence. In the NONE Group, two participants responded below-average confidence. The presence of relevant topics and keywords as cues could both guide or inadvertently influence users' decisions: while they can guide users, any deviation from the suggested keywords or topics might dent their confidence, especially if their labels don't align with these hints. More than half of the NA Group participants rated their confidence as below average. This observation is intriguing; even though automatic evaluation metrics suggest advantages for the NA group over other groups in terms of label quality and time efficiency, there appears to be a gap in user confidence. This discrepancy could lead us to question the efficacy of the NTM. Is it making users more cautious about AI tools, or are its highly specific keyword suggestions causing doubt in users when their decisions deviate?


%% Zongxia

==> sections/999-dregs.tex <==
%% INTRODUCTION
% \jbgcomment{I think the introduction needs to be restructured:

% \begin{itemize}
%     \item First paragraph: going from documents to labels.  Give examples, cite grounded theory.

%     \item Second paragraph: Now you can talk about topic models.  They help give a high level overview.

%     \item Next paragraph can be about active learning, you can mention alto saying that it's not either or, both are helpful.

%     \item Then you can talk about how this hasn't been verified with modern topic models, emphasize that this is a gap in the literature.

%     \item Then give contributions and conclusion of this paper.

% \end{itemize}

% }

% \jbgcomment{This might be confusing to people: they might think you're just doing labeling / classification.  make it clear that this is \emph{establishing} the label set.  Say something like "in contrast to classification, where the label set is known \textit{a priori}"}

% \jbgcomment{Maybe be a little more concrete about examples of label sets that have been created this way?}

% Andrew, Zongxia
% In contrast to classification, where the label set is known \textit{a priori},
Establishing a label set for a collection of documents is a fundamental task
in social science, political science, linguistics,
education, and bioinformatics~\cite{liu2016overview,
paul-girju-2009-topic}. In particular, grounded theory emphasizes
``\textit{structural coding}'' as a framework for discovering similarities and differences in large-scale experimental data, and assigning meaning to it 
\cite{glaser2017discovery, Lindstedt2019, informatics8010019}.
%
For example, \citet{yehia2015} interviewed participants for an \abr{hiv} prevention
clinical trial, and developed a \textit{coding} scheme to group questions
asked into distinct domains, such as \textit{Trial Experience},
\textit{Demographic Information}, etc.~\cite{Namey2007DataRT}. Such a process
is difficult and time-consuming,
% with an increasing amount of online data nowadays, 
in part because it requires both a global understanding of the entire dataset,
and local knowledge to accurately label individual documents.

% In contrast to classification, where the label set is known \textit{a priori}, label set creation requires both a global understanding of the entire dataset...
% Creating a high quality label set is difficult and time-consuming, in part because it requires both a global understanding of the entire dataset, which may be millions of tokens, and local knowledge to accurately label individual documents.

% \jbgcomment{Forward point to later sections with parenthetical notes.  E.g.,
% for the user study, say user study (Section X)}
% \jbgcomment{Can we give more concrete evidence of popularity?  E.g., number of citations, etc.?}

% Topic modeling has emerged as a popular tool that can help with the \textit{coding} process.
% % , with its application across linguistics, education, and other fields~\cite{paul-girju-2009-topic}. 
% The most popular topic model, Latent Dirichlet Allocation (\abr{lda})~\cite{blei2003lda} has over 40,000 citations with numerous extensions and variants~\cite{TMevolution}, such as supervised and neural topic models~\cite{slda, ijcai2021p638}. 

% \jbgcomment{Give a little more information on how active learning helps\dots this depends on the reader knowing that you're doing classification}

% \jbgcomment{perhaps focus more on probabilistic topic models here so that you're setting up a bigger contrast later?}

% \jbgcomment{See style guide on non-breaking spaces}
% \jbgcomment{expand traditional: probabilistic and unsupervised}

Topic modeling~\cite{boyd-graber-17} can help with the
coding process (Section ~\ref{section:background}).
% Topic models facilitate the clustering of documents and the extraction of meaningful themes or topics, which enables professionals like social scientists and legal experts to quickly grasp the semantic landscape of a large corpus~\cite{Lawtopic}. 
The most popular topic model, Latent Dirichlet Allocation (\abr{lda})~\cite{blei2003lda} has over 40,000 citations with numerous extensions and variants~\cite{TMevolution}, such as supervised and neural topic models~\cite{slda, ijcai2021p638}. 
% \abr{lda} is extensively used with a wide range of applications~\cite{Jelodar2019}. 
\abr{lda} treats documents to be mixtures of latent topics, each represented by a distribution over words. 
It mainly serves for the purpose of data exploration, or dimensionality reduction for classification~\cite{blei2003lda}.

Prior research has demonstrated the effectiveness of combining \abr{lda} with a separate active learning classifier to help people create label sets more efficiently~\cite{alto}: topic models provide a global overview of the data,  exposing the broad themes of the corpus that help with creating a label set; active learning selects documents that direct the annotator's attention to topically distinct examples to label, and train the classifier more efficiently.
% However, an open question remains whether \abr{ntm}s, which use continuous text embeddings to capture complex, contextual, and semantic relationships in high-dimensional data, are better for these user-focused tasks.

While prior research has demonstrated the effectiveness of
% active learning and 
traditional topic models like \abr{lda} in accelerating the document labeling process, a gap remains in the literature given recent advancements in topic modeling techniques. 
Neural topic models (\abr{ntm}), which use continuous text embeddings to capture contextual and semantic relationships in high-dimensional data, have gained prominence, often outperforming traditional models on automatic evaluation metrics, such as coherence ~\cite{kitty_ctm}. 
However, automatic evaluation metrics have been called into question, and do not necessarily show a positive correlation between the coherence and human preference on topic model outputs \cite{neuralbroken}. There's a lack of work assessing neural models on their practical applications, such as helping people perform content analysis.

% Topic modeling has emerged as a popular tool that can help with the \textit{coding} process. Classical probabilistic topic model is an unsupervised clustering method that automatically discovers abstract topics, topic keywords of a set of documents using Bayesian Priors~\cite{bayes1763essay}. The most popular topic model, Latent Dirichlet Allocation (\abr{lda})~\cite{blei2003lda} has over 40,000 citations with numerous extensions and variants~\cite{TMevolution}, such as supervised and neural topic models~\cite{slda, ijcai2021p638}. \abr{lda} is extensively used with wide range of applications~\cite{Jelodar2019}. \abr{lda} treats documents to be mixtures of latent topics, each represented by a distribution over words. It mainly serves for the purpose of data exploration, or dimensionality reduction for classification~\cite{blei2003lda}. Prior research demonstrates the effectiveness of \abr{alto} (using \abr{lda} with a separate active learning classifier), help people create label sets more efficiently~\cite{alto}. However, an open question remains whether \abr{ntm}s, which use continuous text embeddings to capture complex, contextual, and semantic relationships in high-dimensional data, are better for these user-focused tasks.


% \jbgcomment{perhaps forward point to where you spell out the debate in more detail later in the paper?}
% \mzcomment{forward point to where I spell out the debate in more detail later in the paper on the above paragraph}

% \jbgcomment{Nowhere do we introduce the name tenor.  Are we not doing that?  Topic Enabled Neural Organization and Recommendation?}

% \jbgcomment{Now or later, give intuition on why these models might be better: they can learn from the labels over time, incorporate world knowledge, etc.  If you don't do it here, forward point to where you do.}

% We aim to study people's judgement and the gap on classical, supervised, and neural topic models in a task based setting, using topic models and active learning to create label sets, and evaluate topic models with both automatic evaluation metrics, and human ratings. Our contributions are:
We aim to fill this gap, and study the performance of neural, supervised, and
classical topic models for accelerating document annotation and label set
creation.  Our contributions can be summarized as follows:
\begin{enumerate*}
    \item We introduce \abr{tenor}, a Topic Enabled Neural Organization and Recommendation system that 
    % modern \abr{ntm} and active learning that 
    helps people to create label sets and annotate documents with the assistance of \abr{ntm}s and active learning. 
    
    \item We provide a human-in-the-loop, task-based evaluation of neural, supervised and classical topic models for document exploration and label set creation. We share the code for the interface, experiments, and data publicly.
    
    \item We run a 60-person user study, and find that people using \abr{tenor} create higher quality label sets than using classical topic models, as measured by cluster metrics (Section ~\ref{user study}).
    % in addition, users using \abr{salto} (supervised topic models and active learning) have a more similar experience with \abr{tenor} than with \abr{alto}. 
    % People using \abr{ntm}s and \abr{slda} rely more on topic model keywords to come up with labels for documents. 
    % where users assess the quality of topic models based on topics, their associated keywords, and the relevance of these keywords to individual documents to create labels.
    

% \jbgcomment{Run style checker script, it will help you remove "We find"}

    % \item The Contextualized Topic Model (\abr{ctm}) \cite{kitty_ctm}, a popular \abr{ntm}, helps users establish a higher quality label set more quickly than classical and supervised topic models; in addition, \abr{ctm} provides better topic features for classification than classical topic models.

    \item We show that automated metrics do not give a complete picture of topic models, and that thoughtfully using topic models as part of a larger system with human interactions gives a more comprehensive understanding of their real-world utility (Section ~\ref{user study}).
    % is important to evaluate topic models on practical tasks.


    

\end{enumerate*}



% Andrew, alto, Zongxia
% Document annotation is a fundamental but labor-intensive task, that often requires manually labeling thousands of examples.  
% such as classification, question answering, and translation.
% Document annotation and label set creation are fundamental tasks in many fields such as social science, law, and biology ~\cite{liu2016overview}. 
% In particular, social science heavily relies on grounded theory and “coding” for content analysis from large-scale online and experimental data~\cite{glaser2017discovery, Lindstedt2019, informatics8010019}. 
% % In particular, social scientists often use topic models to do content analysis from increasing large-scale online, social science, and experiment data~\cite{Lindstedt2019}.
% % Besides exploring datasets, annotation and individual data analysis remain an essential part of the social science research pipeline ~\cite{informatics8010019}. 
% Creating a high quality label set is difficult and time-consuming, in part because it requires both a global understanding of the entire dataset, which may be millions of tokens, and local knowledge to accurately label individual documents.
% % , in addition to requirement of expert level knowledge of the specific dataset. 
% % In addition, data annotation is also an essential part for law field ~\cite{Lawtopic}, and rising field of language models ~\cite{frei2022annotated}. 

% % large language models are fine tuned on labeled passages for improving alignment with human values and conversability (cite RLHF);
% % computational linguistics uses such annotation to determine word senses and sentiment (Kelly
% % and Stone, 1975; Kim and Hovy, 2004); 
% % while social science uses grounded theory and “coding” for content analysis (cite Budge, 2001; Klingemann et
% % al., 2006).
% % Classification takes these labeled data as a training set and labels new data automatically. 
% % TODO: explain "high quality"


% Topic modeling has emerged as a popular tool for content analysis.
% % across multiple disciplines, from law to social sciences to computational linguistics \cite{legaltopic}. 
% It 
% % encapsulate semantic structures and contexts within text data,
% facilitates the clustering of documents and the extraction of meaningful themes or topics. This enables professionals like social scientists and legal experts to quickly grasp the semantic landscape of a large corpus \cite{Lawtopic}. 
% % The evaluation of topic models through human interaction remains an ongoing area of research
% % \cite{2022humancentri\abr{ctm}}.


% Active learning and topic models have been shown to help
% humans annotate documents: Topic models provide a global
% overview of the data, exposing the broad themes of the corpus that help with creating a label set.
% % so users know what labels to create.
% Active learning selects documents for annotation that train the classifier more efficiently
% % and directs the user’s attention locally to them 
% ~\cite{alto}.


% % Zongxia
% % Document annotation is a labor-intensive but crucial task across various domains including law, social sciences, and computer science.
% % For instance, law firms often grapple with the challenge of sifting through, reading, and annotating voluminous sets of documents for each case. The absence of efficient technological solutions can make this task not only mentally exhausting but also time-consuming, compromising the quality of analysis and reasoning. % \cite{LawTech2020}.

% % In addition to topic modeling, active learning plays a vital role in accelerating the process of document labeling~\cite{alto}. Unlike topic models, which offer a broad, global overview of a text corpus, active learning focuses on guiding users' attention to specific documents that are deemed most informative for annotation from a pool of unsorted texts. When integrated with topic models, active learning enables a dynamic human-machine interaction, allowing users to gain both specific (local) and general (global) insights from a corpus. This synergy offers a compelling and nuanced way to engage with topic models.

% While prior research has demonstrated the effectiveness of active learning and traditional topic models like  /abr{lda} in accelerating the document labeling process ~\cite{alto}, a gap remains in the literature given recent advancements in topic modeling techniques. Neural topic models (\abr{ntm}) have gained prominence, often outperforming traditional models on automatic evaluation metrics ~\cite{kitty_\abr{ctm}}. However, there's a lack of work assessing these models on their practical applications, such as helping people perform content analysis.

% We aim to fill this gap, and study the performance of neural, supervised, and classical topic models for accelerating document annotation and label set creation.
% % we evaluate the overall quality of labels created by users for each of the model, then survey on users' experience on labeling documents with topic models, such as keyword coherence, and survey them how much they depend on topic model outputs to create labels. We also propose a new evaluation of topic models that both consider the quality of topics generated, in terms of keywords and topics, and a way evaluating individual documents within each topic. We further analyze the topics and documents generated by different topic models to evaluate their subjective quality.
% % , and plot a correlation between user performance and topics as labels 
% % (or something elase, to plot a correlation between human performance and some other metrics).
% % Zongxia, Andrew
% % \textbf{Contribution}  
% Our contributions can be summarized as follows: 
% \begin{enumerate}
%     \item We provide a human-in-the-loop, application-based evaluation of neural, supervised and classical topic models, using the task of document annotation and label set creation, where users assess the quality of topic models based on topics, their associated keywords, and the relevance of these keywords to individual documents to create labels.

%     \item We find that for the user study, \abr{ntm} helps users produce a higher quality label set more quickly than classical topic models and supervised topic models; in addition, \abr{ntm} provides richer topic information to a classifier for downstream classification task than classical topic models.
%     % This suggests that the \abr{ntm} features either help the classifier better classify documents or suggest better next documents to label.

%     \item We show that automated metrics don't show a complete picture of topic models, and that thoughtfully using topic models with human interactions for specified tasks are important to evaluate topic models on practical tasks.

%     % \item We validate the effectiveness of the Contextualized Topic Model (\abr{ctm}), a popular neural topic model, over traditional  /abr{lda}, in both simulated and real user studies. We show that \abr{ctm} helps users to produce higher quality label sets (according to cluster metrics) more quickly,
%     % and provides better document-level features for automated classification.

%         % (not enough data?) from surveys, we find that users have more confidence in their annotations for classical  /abr{lda}.
        
%     % \item We evaluate the effectiveness of topic model and active learning helping users label documents, find that most users find topic model topics help them come up with labels for documents.

%     % Needs details on the method, how it's novel and valuable; Is this a novel preference function?
%     % \item We introduce a straightforward yet effective method for active learning, facilitating the selection of documents for labeling. Our method also supports partially labeled datasets, which can be leveraged for training topic models and subsequently used to generate approximate labels for the remaining documents.

%     \item We build an interface to label documents with the assistance of topic models and active learning, and run a user study with 60 users. We share the code for the interface, experiments, and data publicly.
%     % , and evaluate the their preference on the topics generated by topic models when doing annotation task.
    

% \end{enumerate}

% 3.  Our evaluation comparing the quality of human-created labels with those generated by LLMs reveals that LLMs, when integrated with active learning and topic modeling techniques, also produce labels of higher quality.


% In a data driven world today, with a set of unlabeled data/documents, there are two main things important to us. The first important thing is we hope to get a classifier that could quickly help us pick documents of possible new labels (labels we have not created) so the classifier can be fitted to more distinct classes that could possibly cover most of the categories in the dataset. Active learning classifier will direct users’ attention locally to documents that lies on the edge of decision boundaries. However, active learning is not always perfect by itself with possible biases on picking which document to label. Topic models has two additional benefits over just active learning under a real user setting. Topic models can provide a quick overview of latent topics over a corpus. The top related keywords will be associated with each topic. With the help of topic models, with a set of unlabeled documents, users can explore potent topics/labels of documents, having a global overview of the set of documents first. The second advantage of topic modeling is to provide extra information to the classifier, which both help a quick gain of purity, rand index, normalized mutual information  in classifier predictions on the rest of the dataset, as well as providing topic diversity information to the classifier, thus reducing bias in document recommendation of the classifier. 

% There has been a gap between evaluation of neural topic models and classical topic models. Human centric or human in-the-loop evaluation are important in the era of data-driven world today. Previous work already shown a effectivenss of combining active learning and traditional topic model ( /abr{lda}) reduces users’ mental stress, frustration level, as well as resulting in a higher quality of the prediction clusters of the classifier on the rest of the dataset with user labels within one hour study session. Within the new gaining and power of pre-trained language models, contextualized topic model is able to use contexual embeddings to generate more specific topic keywords, as well as higher coherence score, and generate document level topic distributions with existing contextual information. We enhance the capabilities of Contextualized Topic Models (\abr{ctm}) to augment classifier performance in active learning settings, while also establishing a comparative evaluation framework that is both human-centric and oriented towards large language models (LLMs)


% With the renaissance of neural networks in recent years, there's an escalating demand for vast amounts of human-labeled textual data across numerous disciplines. Computational linguistic tasks, ranging from sentiment classification and named entity recognition to part-of-speech tagging, hinge on the availability of this massive labeled dataset to optimize model performance. Contemporary large-scale language models, such as GPT-4, rely heavily on a combination of immense unlabeled data sourced from the web and a significant portion of human-annotated data. For instance, the reinforcement learning human feedback (RLHF) employed in training ChatGPT is contingent upon a substantial volume of such labeled data. Beyond computational linguistics, fields like legal systems, political science, and bioinformatics leverage topic modeling extensively to facilitate the creation of label sets for their vast document repositories.  (Less is More paper) states the performance of large language models highly depends on the quality of the dataset over quantity.  The imperative for efficient acquisition of high-quality labels has never been more pronounced than in today's data-driven age. 


%% zongxia


%%END OF INTRODUCTION


% \begin{table*}[th]
%     \centering
% \begin{tabular}{ |p{6cm}||p{6cm}|  }
%  \hline
%  \multicolumn{2}{|c|}{\textbf{Top Keywords}: 20 Newsgroup} \\

%  \hline
%  LDA & CTM\\
%  \hline
%  \underline{Topic~0}: `posting', `host', `computer', `science', `line', `message' & \textcolor{gray}{\underline{Topic~0}: `dengue', `vaccine', `sanofi', `dengvaxia', `phillipines', `vaccination'} \\
%  \underline{Topic~1}: `virus', `countries', `new', `according', `dr', `pandemic' &  \textcolor{gray}{\underline{Topic~1}: `virus', `countries', `new', `according', `dr', `pandemic'} \\ 
%  \underline{Topic~2}: `time', `get', `however', `gonaives', `haiti', `town, `stud' & \textbf{\underline{Topic~2}: `india', `genotype', `denv', `asian', `study', `singapore'}\\
%  \hline
% \end{tabular}

% \caption{Example top topic keywords generated by LDA and ETM for 20 newsgroup dataset}
% \label{tab:example}
% \end{table*}



%%% Insert table of keywords by topic models here

\jbgcomment{instead of saying that the advantages are discussed, preview what the advantages are.}

This section delves into classical and supervised topic models-\abr{slda}, along with the latest \abr{ntm}s. Their advantages are discussed, and we demonstrate how users can use these models for more efficient and higher-quality label set generation. We also introduce active learning, and illustrate how to make it direct users' attention to specific documents and its effectiveness in optimizing classifier predictive accuracy across the dataset.


\subsection{Active Learning}

% Add some background on what active learning is
% When training a classifier with an existing set of labeled data, not every document in the dataset holds equal potential for bolstering model performance. Some documents are inherently richer in information and more informative than others.
Active learning harnesses helps annotators label the documents that will help the classifier the most~\cite{active-learning}. Given a classifier trained on a handful of examples, active learning finds the documents that are most ambiguous---typically those teetering on the boundaries of class definitions. Active learning strategically directs users to annotate these documents. % This approach is invaluable in situations constrained by time or budget, ensuring that the classifier benefits maximally from minimal user input.

\jbgcomment{perhaps cite the ``early gains matter'' paper?}

\subsection{Topic Models}

\jbgcomment{Perhaps we need a transition here: }

Given a substantial corpus $D$ and a specified number of topics $K$, topic models automatically categorize $D$ into $K$ distinct clusters. Each cluster represents a latent topic characterized by a set of representative keywords, which signifies the central theme of that topic. In the following sections, we delve into different kinds of topic models we use in our experiment and user study.


\subsection{Latent Dirichlet Allocation} \label{lda}
Latent Dirichlet Allocation (\abr{lda}) ~\cite{blei2003lda} is a seminal topic modeling approach. \abr{lda} assumes each document to be mixtures of latent topics, each represented by a distribution over words. While exact inference in \abr{lda} is computationally challenging, variational inference is commonly employed to approximate the posterior distributions of the topics within documents. 


\subsection{Supervised Latent Dirichlet Allocation} \label{slda}
\abr{slda} retains the generative process inherent to \abr{lda} but introduces an additional step to incorporate response variables. The initial phase uncovers latent topics in a corpus, then it uses generalized linear models to align these latent topics with the response variables, yielding topics that are representative of the response variable. Take sentiment analysis for an example, \abr{lda} generates topics about what people generally talk about in movie comments dataset, and users have no control on the generated topics. \abr{slda}, on the other hand, can use movie stars as a response variable, and can align topics with star ratings, where the topics and keywords generated are more strongly associated with movie ratings. Users can analyze what people generally talk about for different levels of star ratings. 

% This is where a supervised topic model like \abr{slda} ~\cite{slda} can offer advantages. When an annotator provides labels for a subset of documents within a dataset, sLDA can better align the topic keywords with those pre-existing labels, thereby producing topics that are both more coherent and tailored to the annotator's perspective. Furthermore, as the annotator continues to label documents, the topics can evolve to become increasingly refined. sLDA retains the generative process inherent to LDA but introduces additional steps to incorporate response variables. The initial phase uncovers latent topics in a corpus. Subsequently, generalized linear models align these latent topics with the response variables, yielding topics that not only represent the latent themes but are also predictive of the response variables. In our study, we have adopted classifier predictions as these response variables.


% Background information of NTM to be added. Should we describe all NTMs or just CTM?

% \jbgcomment{I think you can talk generally about all neural models: having a representation for X, Y.  Then focus on CTM as an exemplar}
\subsection{Neural Topic Modeling} \label{etm}
Classical topic models rely on probabilistic graphical models to identify a set of topics based on word co-occurrence statistics. In contrast, \abr{ntm}s use the expressive power of neural networks to capture complex and non-linear relationships in high-dimensional data. This makes \abr{ntm}s capable of capturing more contextually rich and semantically coherent topics. Additionally, neural topic models can be easily integrated with other neural network architectures and can take advantage of pre-trained word embeddings like Word2Vec~\cite{word2vec} or GloVe~\cite{pennington-etal-2014-glove}, which allow them to incorporate semantic information. Current popular \abr{ntm}s include Bertopic ~\cite{bertopicMark}, Embedded topic model (\abr{etm}) ~\cite{ETMtopic}, contexualized topic model (\abr{ctm}) ~\cite{kitty_CTM}. Specifically, \abr{ctm} is takes advantage of contextual word embeddings to enhance the quality of discovered topics. Unlike standard topic models that consider each word as an isolated unit, \abr{ctm} understands the context in which a word appears in the document, resulting in more coherent and semantically meaningful topics. It usually leverages pre-trained language models like BERT to generate contextual embeddings, which serve as input features for the topic model.

% \mzcomment{Will need to reduce the background and methodlogy section to include related work}


